A radio transient with unusually slow periodic emission

The high-frequency radio sky is bursting with synchrotron transients from massive stellar explosions and accretion events, but the low-frequency radio sky has so far been quiet beyond the Galactic pulsar population and the long-term scintillation of AGN. The low-frequency band, however, is sensitive to exotic coherent and polarised radio emission processes such as electron cyclotron maser emission from flaring M-dwarfs [1], stellar magnetospheric plasma interactions with exoplanets [2], and a population of steep-spectrum pulsars [3], making Galactic plane searches a prospect for blind transient discovery. Here we report an analysis of archival low-frequency radio data that reveals a periodic, low-frequency radio transient. We find that the source pulses every 18.18 minutes, an unusual periodicity not previously observed. The emission is highly linearly polarised, bright, persists for 30--60 s on each occurrence, and is visible across a broad frequency range. At times the pulses comprise short ($<0.5$-s) duration bursts; at others, a smoother profile is observed. These profiles evolve on timescales of hours. By measuring the dispersion of the radio pulses with respect to frequency, we have localised the source to within our own Galaxy, and suggest that it could be an ultra-long period magnetar.

==> preamble.tex <==
%MNRAS style
\newcommand{\fig}{Fig.}
\newcommand{\figs}{Figs.}
\newcommand{\Fig}{Fig.}
\newcommand{\EFig}{Extended Data Fig.}
\newcommand{\Figs}{Figs.}
\newcommand{\sect}{Section}
\newcommand{\sects}{Sections}
\newcommand{\Sect}{Section}
\newcommand{\Sects}{Sections}
\newcommand{\tab}{Table}
\newcommand{\tabs}{Tables}
\newcommand{\Tab}{Table}
\newcommand{\Tabs}{Tables}
\newcommand{\eqn}{equation}
\newcommand{\eqns}{equations}
\newcommand{\Eqn}{Equation}
\newcommand{\Eqns}{Equations}
\newcommand{\etal}{et~al.}

\newcommand{\farcm}{\mbox{\ensuremath{.\mkern-4mu^\prime}}}%    % fractional arcminute symbol: 0.'0
\newcommand{\farcs}{\mbox{\ensuremath{.\!\!^{\prime\prime}}}}%  % fractional arcsecond symbol: 0.''0
\newcommand{\fdg}{\mbox{\ensuremath{.\!\!^\circ}}}%             % fractional degree symbol:     0.°0

% Source name
\newcommand{\src}{GLEAM-X\,J\,162759.5-523504.3}
% Dispersion measure
\newcommand{\srcDM}{\ensuremath{57}}
\newcommand{\DMerror}{\ensuremath{1}}
\newcommand{\DMunit}{pc\,cm\ensuremath{^{-3}}}
% Rotation measure
\newcommand{\srcRM}{\ensuremath{-61}}
\newcommand{\RMerror}{\ensuremath{1}}
\newcommand{\RMunit}{rad\,m\ensuremath{^{-2}}}
% Period
\newcommand{\srcPlong}{\ensuremath{1091.1690}}
\newcommand{\srcPerr}{\ensuremath{0.0005}}
\newcommand{\srcP}{\ensuremath{1091}}
% Spectral index
\newcommand{\srcalphaerr}{\ensuremath{0.04}}
\newcommand{\srcalpha}{\ensuremath{-1.16}}

\newcommand{\ndetections}{71}
% Period derivative
\newcommand{\srcPdot}{\ensuremath{6\times10^{-10}}}
\newcommand{\Pdotunit}{\,s\,s\ensuremath{^{-1}}}
% Other
\newcommand{\ergpers}{erg\,s\ensuremath{^{-1}}}
